No star is good news: A unified look at rerandomization based on $p$-values from covariate balance tests

Modern social and biomedical scientific publications require the reporting of covariate balance tables with not only covariate means by treatment group but also the associated $p$-values from significance tests of their differences. The practical need to avoid small $p$-values renders balance check and rerandomization by hypothesis testing standards an attractive tool for improving covariate balance in randomized experiments. Despite the intuitiveness of such practice and its arguably already widespread use in reality, the existing literature knows little about its implications on subsequent inference, subjecting many effectively rerandomized experiments to possibly inefficient analyses. To fill this gap, we examine a variety of potentially useful schemes for rerandomization based on $p$-values (ReP) from covariate balance tests, and demonstrate their impact on subsequent inference. Specifically, we focus on three estimators of the average treatment effect from the unadjusted, additive, and fully interacted linear regressions of the outcome on treatment, respectively, and derive their respective asymptotic sampling properties under ReP. The main findings are twofold. First, the estimator from the fully interacted regression is asymptotically the most efficient under all ReP schemes examined, and permits convenient regression-assisted inference identical to that under complete randomization. Second, ReP improves not only covariate balance but also the efficiency of the estimators from the unadjusted and additive regressions asymptotically. The standard regression analysis, in consequence, is still valid but can be overly conservative.

==> cmdlist_PA.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\
\def\fall{\text{for all} \ }
\def\mj{\mathcal J}
\def\rw{{\red with }}
\def\bbw{{by }}
\def\matd{\ma_{\ts,\dmd}}
\def\dmd{\diamond}
\def\gray{\color{gray}}
\def\black{\color{black}}
\def\pvbs{{\red $p$-value-based/hypothesis testing-based }}
\def\htbs{{hypothesis testing-based }}
\def\dgp{data-generating process}
\def\rep{ReP}
\def\reps{{ReP }}
\def\repsch{ReP schemes}
\def\repschs{{ReP schemes }}
\def\schreps{{schemes for ReP }}
\def\schrep{{schemes for ReP}}


\def\me{\mathcal E}
\def\meo{\me_1}
\def\met{\me_2}
\def\meth{\me_3}
\def\mrm{\mr^{m}}
\def\mrjq{\mr^{(J+1)(Q-1)}}
\def\hses{\hse_*}
\def\mb{\mathcal B}
\def\lmlr{logistic and {\mlr} }
\def\lmlrs{logistic and {\mlr}s }
\def\hst{H^*}
\def\hsti{(H^*)^{-1}}
\def\oh{1_{|H'|}}
\def\tbb{\tilde{\bm \beta}}
\def\gci{Gaussian correlation inequality}
\def\gcis{Gaussian correlation inequality }
\def\mr{\mathbb R}
\def\mra{\mr(a)}
\def\mac{\ma^c}
\def\mc{\mathcal C}
\def\htxj{\htau_{x,j}}
\def\fort{\qquad\text{for} \ \ }
\def\wheret{\qquad\text{where} \ \ }
\def\qj{{\qiqp; \ \jej}}
\def\tresch{\tres schemes}
\def\btb{\tilde{\bm\beta}}
\def\malogitjt{\ma_{\logit, \jt}}
\def\malogitmg{\ma_{\logit, \m}}
\def\malogitcs{\ma_{\logit, \css}}

\def\malmjt{\ma_{\lm, \jt}}
\def\malmmg{\ma_{\lm, \m}}
\def\malmcs{\ma_{\lm, \css}}

\def\matjt{\ma_{\ts, \jt}}
\def\matmg{\ma_{\ts, \m}}
\def\matcs{\ma_{\ts, \css}}

\def\mafmg{\ma_{\ff, \m}}

\newcommand{\tbt}{\tb^\T}
\def\hg{\hat\gamma}
\def\hgz{\hg_0}
\def\hgo{\hg_1}
\def\hvl{\hat v_\lin}
\def\hcs{\hat c_*}
\def\hcf{\hat c_\fisher}
\def\hcn{\hat c_\neyman}

\def\tbq{\tilde{\bm \beta}_q}
\def\ao{\bm a_1}
\def\aqmo{\bm a_{Q-1}}
\def\aq{\bm a_q}
\def\teq{\trianglelefteq}
\def\wiq{\mi_{iq}}
\def\wiqq{\mi_{iQ}}
\def\wio{\mi_{i1}}
\def\qp{Q_\pluss}
\def\qeq{q= \ot{Q}}
\def\byqp{\by(q')}
\def\th{\theta}
\def\hyg{\hy_\gamma}
\def\hbt{\hb^\T}
\def\htxt{\htx^\T}
\def\pzmo{p_{0,\x}}
\def\pjmo{p_{j, \x}}
\def\svxinvinv{\sigma(\vx^{-1})^{-1}}
\def\svxinv{\sigma(\vx)^{-1}}
\def\shoinv{\sigma(\ho)^{-1}}
\def\shvinv{\sigma(\hv)^{-1}}
\def\stvinv{\sigma(\tv)^{-1}}

\def\mqp{\mq_\pluss}
\def\oo{o(1)}
\def\wmlr{W_\textup{\mlogit}}
\def\wmlogit{\wmlr}
\def\tbqj{\tb_{qj}}
\def\tmlogit{T_{\mlogit}}
\def\sumiq{\sum_{i:Z_i = q}}
\def\tlm{T_\lm}
\def\tfor{\qquad\text{for} \ \ }
\def\twhere{\qquad\text{where} \ \ }
\def\chisq{\chi^2}
\def\llrt{\lambda_{\lrt}}
\def\rp{R_\pluss}
\def\emo{e_{Q-1}}
\def\eo{e_1}
\def\hxt{\hx^\T}
\def\premlogit{Assume a completely randomized experiment with $Q \geq 2$ treatment arms and Conditions \ref{asym} and \ref{cond:glm_Q}.}
\def\mlesss{{{\mle}s }}
\def\ha{H_\text{a}}
\def\ths{\theta^*}
\def\mq{\mathcal Q}
\def\eq{e_q}
\def\eqq{e_Q}
\def\thq{\theta_q}
\def\thqq{\theta_Q}
\def\thqmo{\theta_{Q-1}}
\def\bqz{\beta_{q0}}
\def\bqzs{\beta_{q0}^*}
\def\tbqz{\tb_{q0}}
\def\sumqmo{\sum_{\qiqp}}
\def\marem{\ma_\textup{rem}}
\def\mamgt{\ma_\mgt}
\def\majtt{\ma_\jtt}
\def\macst{\ma_\cst}

\def\pluss{{\scaleto{+}{4.5pt}}}
\def\tbn{\tb_0}
\def\tthn{\tilde\theta_0}
\def\maf{\ma_\textup{f}}
\def\qiqp{q\in\mqp}\def\qeqmo{q = \ot{Q-1}}
\def\mqp{\mathcal Q_\pluss}
\def\qiq{q\in\mq}
\def\jej{j = \ot{J}}
\def\jij{j \in\{ \ot{J}\}}
\def\meani{N^{-1}\sumi}
\def\byz{\by(z)}
\def\byq{\by(q)}
\def\mamodr{\ma_{\x, \dr}}
\def\mamojt{\ma_{\x, \jt}}
\def\mamocs{\ma_{\x, \css}}
\def\mamomg{\ma_{\x, \m}}

\def\drt{{\textup{t}, \dr}}
\def\madrt{\ma_\drt}
\def\drs{\dr=\jt, \m, \css}
\def\dg{\dagger}
\def\mgt{{\textup{t}, \m}}
\def\jtt{{ \textup{t}, \jt}}
\def\cst{{\textup{t}, \css}}
\def\epj{\ep_{[J]}}
\def\yiz{Y_i(z)}
\def\yiq{Y_i(q)}
\def\fl{* = \fisher, \lin}
\def\hgs{\hat\gamma_*}
\def\succi{\succeq_\infty}
\def\wlssub{\textup{wls}}
\def\piki{\pi_\ki}
\def\pik{\pi_\sk}
\def\moo{M_{11}}
\def\btt{B_{22}}
\def\bot{B_{12}}
\def\mtt{M_{22}}
\def\mot{M_{12}}

\def\mooi{M_{11, \infty}}
\def\btti{B_{22,\infty}}
\def\boti{B_{12,\infty}}
\def\mtti{M_{22,\infty}}
\def\moti{M_{12,\infty}}

\def\bX{\bar X}
\def\btx{\left\{\hb^\T(\xki-\bxk )\right\}}
\def\xtb{\left\{(\xki-\bxk )^\T\hb\right\}}
\def\nkinv{N_\sk^{-1}}
\def\sumki{\sumk\sumink}
\def\sumink{\sum_{i=1}^\nk}
\def\rssk{\textsc{rss}_\sk}
\def\he{\hat\epsilon}
\def\heki{\he_\ki}
\def\blue{\color{blue}}
\def\red{\color{red}}


\def\tre{{TRe}}
\def\tres{{TRe }}
\def\szinv{S_0^{-1}}
\def\hxk{\hat x_\sk}
\def\hmuk{\hat\mu_\sk}
\def\bxk{\bx_\sk}
\def\bxo{\bx_\so}
\def\bxK{\bx_\sK}
\def\plim{\textup{p$\lim$\,}}
\def\imat{G}

\def\vari{\var_\infty}
\def\vsk{v_{*[k]}}
\def\lrt{\textsc{lrt}}
\def\lrts{{\textsc{lrt} }}

\def\vbinv{V_\beta^{-1}}
\def\vb{V_\beta}
\def\szzk{ S_{Z[k]}^2}
\def\sxxk{S^2_{x[k]}}
\def\sxxd{S^2_{x[\cdot]}}
\def\sxzk{S_{xZ[k]}}
\def\htsk{\htau_{*[k]}}
\def\htxk{\htau_{x[k]}}
\def\csk{c_{*[k]}}
\def\vxk{v_{x\sk}}

\def\tk{\tau_\sk}
\def\wk{\omega_{[k]}}
\def\wo{\omega_{[1]}}
\def\wK{\omega_{[K]}}
\def\beginp{\begin{pmatrix}}
\def\endp{\end{pmatrix}}

\def\nzzk{N_{z[k]}}
\def\ezzk{e_{z[k]}}
\def\eok{e_{1[k]}}
\def\ezk{e_{0[k]}}
\def\eoo{e_{1[1]}}
\def\ezo{e_{0[1]}}
\def\eoK{e_{1[K]}}
\def\ezK{e_{0[K]}}

\def\noo{N_{1[1]}}
\def\nok{N_{1[k]}}
\def\nokinv{\nok^{-1}}
\def\noK{N_{1[K]}}

\def\no{{N_{[1]}}}
\def\nK{{N_{[K]}}}

\def\so{{[1]}}
\def\st{{[2]}}
\def\sk{{[k]}}
\def\sK{{[K]}}
\def\nk{{N_{[k]}}}

\def\xki{x_\ki}
\def\ski{s_\ki}
\def\zki{Z_\ki}

\def\ki{{[k]i}}
\def\ts{{\textup{t}}}
\def\ttts{{\texttt{t}}}
\def\ttt{{\texttt{ttest}}}
\def\lmt{\texttt{lm}}
\def\glmt{\texttt{logit}}
 \def\tts{T_{\ts}}

\def\glm{\textup{logit}}
\def\lm{\textup{lm}}
\def\logit{\textup{logit}}
\def\logitt{\texttt{logit}}
\def\mlogit{\textup{logit}}
\def\mlogitt{\texttt{logit}}
\def\qmo{{Q-1}}
%%%%%%%%%%


\def\sxyz{S_{xY(z)}}
\def\gf{\gamma_\fisher}
\def\sumk{\sum_{k=1}^K}
\def\mtf{\mt_\ff }
\def\temp{\delta}
\def\nf{* = \neyman, \fisher}
\def\nfl{* = \neyman, \fisher, \lin}
\def\epm{\ep_{\textup{lm}}}
\def\mtm{\mt_{\textup{lm}}}
\def\gp{\gamma_\textsc{f}}
\def\dd{\sigma(\vxinv)}
\def\pjx{p_{j,\x}}
\def\pjt{p_{j,\ts}}
\def\pzt{p_{0,\ts}}
\def\pjlm{p_{j,\lm}}
\def\pzlm{p_{0,\lm}}
\def\pjglm{p_{j,\logit}}
\def\pjlogit{p_{j,\logit}}
\def\pzglm{p_{0,\logit}}
\def\hsx{\hat S^2_x}
\def\hsxj{\hat S^2_{x,j}}

 \def\vxm{V_{x\pluss}}
 \def\hxm{\hx_\pluss}
 
  \def\vxp{V_{x\pluss}}
 \def\hxp{\hx_\pluss}
 
\def\Vx{V_x}
\def\ff{\textup{f}}
\def\ajf{a_{j,\ff}}
\def\phiinv{\Phi^{-1}}
\def\linv{\phiinv}
\def\ft{\texttt{F}}
\def\moiq{\x \in\{ \ft,  \glmt\}}

\def\txbi{\tx_i^\T\theta}

\def\mlr{{multinomial logistic regression}}
\def\mlrs{{multinomial logistic regression }}
\def\mmlr{{Multinomial logistic regression}}
\def\mmlrs{{Multinomial logistic regression }}
\def\dsim{\stackrel{\cdot}{\sim}}
\def\hys{\hat Y_*}
\def\by{\bar Y}
\def\sumqi{\sumq \sum_{i:Z_i = q}}
\def\sxj{\sxxj}
\def\hxj{\hx_j}
\def\pq{e_q}
\def\hyn{\hy_\nm}
\def\hyf{\hy_\fisher}
\def\hyl{\hy_\lin}
\def\bbr{\mathbb R}
 
\def\epf{\ep_\textup{f}}
\def\sxyq{S_{xY(q)}}
\def\hy{\hat Y}
\def\pjf{p_{j, \textup{f}}}
\def\pjg{p_{j, \logit}}
\def\pqjg{p_{qj, \mlogit}}
\def\pqjmlr{p_{qj, \mlogit}}
\def\tqjmlr{t_{qj, \mlogit}}
\def\pzmlr{p_{0, \mlogit}}
\def\pzg{p_{0, \glm}}
\def\stx{S^2_{\tx}}
\def\xs{{(\x)}}
\def\phim{\phi_\m}
\def\phij{\phi_\jt}
\def\phic{\phi_\css}
\def\phij{\phi_\jt}
\def\phixc{\phi^{(\x)}_\css}
\def\phixm{\phi^{(\x)}_\m}
\def\phixj{\phi^{(\x)}_\jt}
\def\mhls{Mahalanobis}
\def\tX{\tilde X}
\def\methodst{\ttt, \lmt, and \glmt}
\def\wt{W_\ts}
\def\wlm{W_\lm}
\def\wglm{W_\glm}
\def\wlogit{W_\logit}
\def\tjt{t_{j,\ts}}
\def\tjlm{t_{j,\lm}}
\def\tjglm{t_{j,\glm}}

\def\mhl{{Mahalanobis }}
\def\Bm{\|B\|_\mm}
\def\Bpm{\|B'\|_\mm}
\def\mm{{\scaleto{\mathcal{M}}{4pt}}}
\def\dv{\{\sigma(v)\}^{-1}}
\def\ppinv{(\pp)^{-1}}
\def\ppinvsq{(\pp)^{-2}}
\def\moi{\x \in\{ \textup{t}, \lm, \logit\}}
\def\mos{\x = \textup{t}, \lm, \logit}


\def\dri{\dr\in\{\m, \jt, \css\}}
\def\reg{\textup{ReG}}
\def\vl{v_\lin}
\def\vf{v_\fisher}
\def\vn{v_\nm}

\def\phid{\phi_\dr}
\def\dr{\diamond}
\def\m{\textup{mg}}
\def\jt{\textup{jt}}
\def\css{\textup{cs}}

\def\hs{\hat\Sigma}
\def\sigi{\Sigma_\infty}
\def\x{\dg}
\def\vsi{V_\Psi}
\def\on{\Omega_{\neyman}}
\def\os{\Omega_{*}}
\def\cs{c_{*}}
\def\oni{\Omega_{\neyman}}
\def\osi{\Omega_{*}}
\def\csi{c_{*}}
\def\cfi{c_{\fisher}}
\def\cni{c_{\nm}}
\def\cli{c_{\lin}}
\def\lsf{l_{*,\x}}
\def\hsig{\hat\Sigma}
\def\yy{{model} }
\def\rs{\rightsquigarrow}
\def\nn{N_0N_1}
\def\pp{e_0e_1}
\def\si{\Sigma_{\infty}}
\def\sqrtn{\sqrt N}
\def\hts{\htau_*}
\def\begini{\begin{itemize}}
\def\endi{\end{itemize}}
\def\begine{\begin{enumerate}}
\def\ende{\end{enumerate}}
\def\mU{\mathcal{U}}
\def\ep{\epsilon}
\def\dx{D}
\def\hgl{\hg_\lin}
\def\vxx{\vx}
\def\th{\theta}
\def\vi{v_\infty}
\def\rsi{c_{*,\infty}}
\def\rfi{c_{\fisher}}
\def\rni{c_{\neyman}}
\def\vni{v_{\neyman}}
\def\vxi{v_{x}}
\def\ho{\hat\Omega}
\def\hsj{\hat\sigma_j}
\def\tsj{\tilde\sigma_j}
\def\mi{\mathcal{I}}
\def\mgi{\mg_\infty}
\def\mg{\mathfrak{G}}
\def\vxxinv{\vxx^{-1}}
\def\vxinv{\vx^{-1}}
\def\vxiinv{\vxi^{-1}}
\def\vx{v_x}
\def\pd{\partial}
\def\as {\text{a.s.}} 
\def\hth{\hat\theta}
\def\tth{\tilde\theta}

\def\xxx{{consensus }}
\def\xxxs{{consensus}}
\def\rss{\textsc{rss}}
\def\df{\textup{df}}
\def\qt{\textup{qt}}
\def\xx{{decision }}
\def\tx{\tilde x}
\def\tb{\tilde\beta}
\def\xij{x_{ij}}

\def\tbrs{{test-based rerandomization }}
\def\rrs{{rerandomization }}
\def\rr{{rerandomization}}
\def\mle{\textsc{mle}}
\def\mles{{\textsc{mle} }}
\def\vxiinvj{(\vxiinv)_{jj}}
\def\dhb{D_{\hb}}
\def\thb{T_{\lm}}
\def\ttb{T_\glm }
\def\hts{\htau_*}
\def\hd{\hat\delta}
\def\tv{\tilde V}

\def\hv{\hat V}
\def\mn{\mathcal{N}}
\def\li{\mathcal{L}_\infty}
\def\sx{S_x}
\def\sxz{S_{xZ}}
\def\se{\textup{se}}
\def\neyman{\textsc{n}}
\def\rtn{\sqrt N}
\def\htN{\hat\tau_\nm}
\def\htxj{\hat\tau_{x,j}}
\def\tse{\tilde{\textup{se}}}
\def\hse{\hat{\textup{se}}}

\def\htsej{\htxj / \hse_j}
\def\ttsej{\htxj / \tse_j}

\def\sxxinv{(\sxx)^{-1}}
\def\sxxj{S^2_{x,j}}
\def\sxqj{S_{xZ,j}}
\def\szz{S_{Z}^2}
\def\fwlc{The Frisch--Waugh--Lovell theorem}
\def\fwl{the Frisch--Waugh--Lovell theorem}
\def\tsesqj{{(\hse'_j)}^2}
\def\hsesq{\hat{\textup{se}}^2}

\def\txi{\tx_i}
\def\txit{\tx_i^\T}
 
\def\htt{\hat t}
\newcommand{\qxx}{\hat S_x^2}
\newcommand{\qxy}{\hat S_{xY}}
\newcommand{\hgf}{\hat\gamma_\fisher}
\newcommand{\hglo}{\hat\gamma_{\lin,1}}
\newcommand{\hglz}{\hat\gamma_{\lin,0}}
\newcommand{\hglq}{\hat\gamma_{\lin,q}}

\newcommand{\htf}{\hat\tau_\fisher}
\newcommand{\htl}{\hat\tau_\lin}
\def\hts{\hat\tau_*}
\newcommand{\htlsr}{\htl/\tse_\lin}
\newcommand{\htn}{\hat\tau_\nm}

\def\Zi{Z_i}
\def\Yi{Y_i}
\def\sumi{\sum_{i=1}^N}
\def\sumN{\sum_{i=1}^N}
\def\sp{supplementary material}
\def\rank{\textup{rank}}
\def\hbqr{\hb_{q,\ri}}
\def\di{\mathcal{D}_\infty}
\def\ri{\textup{ri}}
\def\htgz{\htau_{\Gamma,z}}
\def\gq{\gamma_q}
\def\q{{[Q]}}
\def\bq{\bm \beta_q}
\def\ml{\mathcal{L}}
\def\ttg{\tbt_\Gamma}
\def\dhtg{\Delta\htg }
\def\dttg{\Delta \ttg}
\def\vttPl {V_{\tau\tau,\lambda}^\|}
\def\vttRl {V_{\tau\tau,\lambda}^\perp}
\def\vttPld {V_{\tau\tau,\lambda}^\| |_{\hd}}
\def\vttRld {V_{\tau\tau,\lambda}^\perp |_{\hd}}
\def\vttPd {V_{\tau\tau,\delta}^\|}
\def\vttRd {V_{\tau\tau,\delta}^\perp}
\def\muzg{ \mu_{0,\Gamma}}



\def\ei{E_\infty}
\def\covi{\cov_\infty}

\def\hz{\hat z}
\def\malw{\mathcal{A}_{\lambda_w,a}}
\def\mal{\mathcal{A}_{\lambda,a}}

\def\dht{\Delta\htau}
\def\dtt{\Delta\tbt}
\def\mlh {\mathcal{D}_\infty (\dht ) }
\def\mlhd {\mathcal{D}_\infty (\dht -\mu_0  \mid \hd ) }
\def\mlha {\mathcal{D}_\infty (\dht \mid \mathcal{A} ) }
\def\mlhad {\mathcal{D}_\infty (\dht  - \mu_0 \mid \mathcal{A}, \hd ) }
\def\mlt {\mathcal{D}_\infty (\dtt ) }
\def\mltd {\mathcal{D}_\infty (\dtt  \mid \hd ) }
\def\mlta {\mathcal{D}_\infty (\dtt  \mid \mathcal{A} ) }
\def\mltad {\mathcal{D}_\infty (\dtt  \mid \mathcal{A}, \hd ) }

\def\mlhtg {\mathcal{D}_\infty (\dhtg  ) }
\def\mlhtgd {\mathcal{D}_\infty (\dhtg - {\red \mu_{0,\Gamma} } \mid \hd ) }
\def\mlhtga {\mathcal{D}_\infty (\dhtg   \mid \mal ) }
\def\mlhtgad {\mathcal{D}_\infty (\dhtg  - {\red \mu_{0,\Gamma} }   \mid \mal, \hd ) }
\def\mlttg {\mathcal{D}_\infty (\dttg  ) }
\def\mlttgd {\mathcal{D}_\infty (\dttg   \mid \hd ) }
\def\mlttga {\mathcal{D}_\infty (\dttg   \mid \mathcal{A} ) }
\def\mlttgad {\mathcal{D}_\infty (\dttg   \mid \mathcal{A}, \hd ) }

\def\mltb {\mathcal{D}_\infty (\dtt  \mid \mathcal{B} ) }
\def\mlyx {\mathcal{D}_\infty (Y  \mid X) }
\def\mly  {\mathcal{D}_\infty (Y  ) }
\def\mltbd {\mathcal{D}_\infty (\dtt  \mid \mathcal{B}, \hd ) }



\def\hd{\hat\delta}
\def\htg{\htau_\Gamma}
\def\sm{{Supplementary Material}}
\def\rem{{ReM }}
\def\rems{ReM}
\def\summ{\sum_{m=1}^M}
\def\tG{\tilde G}
\def\hg{\hat\gamma}
\def\mgq{\mathcal{G}^*}
\def\ma{\mathcal{A}}
\def\tr{\text{tr}}
 
\def\sxx{S^2_x}
\def\dxx{D^2}
\def\htx{\htau_x}
\def\sxq{S_{xq}}
\def\sqx{S_{qx}}
\newcommand{\syx}{ S_{Y x}}
\newcommand{\sxy}{ S_{ x Y}}

\def\ms{* = \nm, \fisher,\lin}
%%%%%%%%%%%%%%%%%%%%
\def\hyf{\hY_\fisher}
\def\hyl{\hY_\lin}
\def\olss{{\textsc{ols}}}
\def\ols{{\textsc{ols} }}
\def\wlss{{\textsc{wls} }}
\def\hb{\hat\beta }
\def\hbf{\hat\beta_\fisher }
\def\hbl{\hat\beta_\lin}

\def\olsf{\ols_\fisher}
\def\olsl{\ols_\lin}
\newcommand{\htau}{ \hat\tau}
\def\htf{ \hat\tau_\fisher}
 
 

\def\hlw{\hat\lambda_\w}
\def\hw{\hat\w}
\def\hx{\hat x}
\def\hX{\hat X}
\def\bx{\bar x}

\def\w{w}
\def\hw{\hat\w}
\def\bw{\bar\w}
\newcommand{\vttw}{  V_{\tau\tau} |_{\hbd}}
\newcommand{\vtlw}{  V_{\tau\lambda} |_{\hbd}}
\newcommand{\vltw}{  V_{\lambda\tau} |_{\hbd}}
\newcommand{\vllw}{  V_{\lambda\lambda} |_{\hbd}}

\newcommand{\vtlwC}{  V_{\tau\lambda} |_{\hbdC}}
\newcommand{\vltwC}{  V_{\lambda\tau} |_{\hbdC}}
\newcommand{\vllwC}{  V_{\lambda\lambda} |_{\hbdC}}
\newcommand{\vttz}{  V_{\tau\tau} |_{\hdz }}
\def\vtwz{  \vtw |_{\hdz }}
\def\vwtz{  \vwt  |_{\hdz }}
\newcommand{\vwwBz}{  \vww |_{\hdz }}
\newcommand{\vwt}{ V_{\w\tau}}
\newcommand{\vtw}{ V_{\tau \w}}
\newcommand{\vww}{ V_{\w\w}}
\newcommand{\vdd}{ V_{\delta\delta}}
\newcommand{\vzz}{ V_{zz}}
\newcommand{\SigWW}{ \Sigma_{ W}}

\newcommand{\vzw}{ V_{z\w}}
\newcommand{\vwz}{ V_{\w z}}
\newcommand{\vzt}{ V_{z\tau}}
\newcommand{\vtz}{ V_{ \tau z}}

\def\htw{\hat{\tau}_w }




\def\mt{\mathcal{T}}
\newcommand{\Dt}{\tbD_{\bt}}
\newcommand{\Dmu}{\tbD_{\mu}}
\newcommand{\Da}{\tbD_{\ba}}
\newcommand{\bC}{ \bm C}

\newcommand{\hba}{\hat{\ba}}
\newcommand{\hbv}{\hat{ \nu}}
\newcommand{\mN}{\mathcal{N}}

\newcommand{\bCq}{\bC_\Q}
\newcommand{\hbo}{\hat\bo}
\newcommand{\bo}{ \Omega}




\newcommand{\Op}{O_{P}(1)}
\newcommand{\op}{o_{P}(1)}
\newcommand{\Q}{\textsc{q}}
 

\newcommand{\hbV}{ \hat{ V}}

\newcommand{\sww}{ S_{ w  w}}
\newcommand{\vlsinter}{\hat{ V}_{\lin}}
\newcommand{\vlsadj}{\hat{ V}_{\fisher}}

\newcommand{\vlsl}{\hat{ V}_{\lin}}
\newcommand{\vlsfols}{\hat{ V}_{\fisher,\ols}}
\newcommand{\vlsfwls}{\hat{ V}_{\fisher,\wls}}


\newcommand{\tbtQ}{\tilde{ \tau}^*}
\newcommand{\hbtQ}{\hat{ \tau}_\Q}

\newcommand{\hbgadj}{\hat{\gamma}_\textsc{f}}


\newcommand{\bG}{ G}
\newcommand{\tbY}{\tilde{ Y}}


\newcommand{\vyy}{ V_{YY}}

\newcommand{\syw}{ S_{Y w}}
\newcommand{\swy}{ S_{ w Y}}
\newcommand{\hbU}{\hat { U}}


\newcommand{\bPi}{ \Pi}
\newcommand{\bPinv}{ \Pi^{-1}}
\newcommand{\bP}{ P}
\newcommand{\bR}{ R}
\newcommand{\Ptwo}{ P_{( G^\perp)}}


\newcommand{\hxi}{\hx_{2:Q}}
\newcommand{\hbWi}{\hbW_{2:Q}}
\newcommand{\bri}{ r_{2:Q}}
\newcommand{\bRi}{ R_{2:Q}}


\newcommand{\bgamma}{ \Gamma}



\newcommand{\bmun}{ \mu_\nm}
\newcommand{\bmuf}{ \mu_\fisher}
\newcommand{\bmus}{ \mu_*}



\newcommand{\lin}{\textsc{l}}
\newcommand{\nm}{\textsc{n}}

\newcommand{\hbts}{\hbt_*}
\newcommand{\hbtf}{\hbt_\textsc{f}}
\newcommand{\hbtn}{\hbt_\textsc{n}}
\newcommand{\hbtl}{\hbt_\textsc{l}}
\newcommand{\bg}{  \gamma }


\newcommand{\hbd}{\hat{\delta}}
\newcommand{\hbdg}{\hbd_g}
\newcommand{\hbdG}{\hbd_G}
\newcommand{\hbdO}{\hat{\delta}^{( O)}}
\newcommand{\hbdX}{\hat{\delta}^{( X)}}
\newcommand{\hbdC}{\hat{\delta}( C)}
\newcommand{\hbdT}{\hat{\delta}^{( \Theta)}}
\newcommand{\hl }{\hat{\lambda}}
\newcommand{\hbdh}{\hbd_h}



\newcommand{\vddG}{ V_{\delta\delta, G}}
\newcommand{\vll}{ V_{\lambda\lambda}}
\newcommand{\vdl}{ V_{\delta\lambda}}
\newcommand{\vld}{ V_{\lambda\delta}}
\newcommand{\vddC}{ V_{\delta\delta}^{( C)}}
\newcommand{\vddCB}{ V_{\delta\delta}^{( C,  B)}}
\newcommand{\vddQB}{ V_{\delta\delta}^{(\cs,  B)}}

\newcommand{\vtd}{ V_{\tau\delta}}
\newcommand{\vtds}{ V_{\tau\delta,*}}
\newcommand{\vtdf}{ V_{\tau\delta,\fisher}}
\newcommand{\vtdn}{ V_{\tau\delta,\textsc{n}}}


\newcommand{\vdts}{ V_{\delta\tau,*}}

\newcommand{\vdtf}{ V_{\delta\tau,\fisher}}
\newcommand{\vdtn}{ V_{\delta\tau, \textsc{n}}}

\newcommand{\vtdG}{ V_{\tau\delta}}
\newcommand{\vtdO}{ V_{\tau\delta}^{( O)}}
\newcommand{\vtdQ}{ V_{\tau\delta}^{\cs}}
\newcommand{\vtdC}{ V_{\tau\delta}^{( C)}}
\newcommand{\vtl}{ V_{\tau\lambda}}
\newcommand{\vtdT}{ V_{\tau\delta}^{( \Theta)}}

\newcommand{\vlt}{ V_{\lambda\tau}}
\newcommand{\vdtG}{ V_{\delta\tau,G}}
\newcommand{\vdtC}{ V_{\delta\tau}^{( C)}}
\newcommand{\vdt}{ V_{\delta\tau}}


\newcommand{\sumn}{\sum_{i=1}^N}
\newcommand{\sumq}{\sum_{q\in\mq}}
\newcommand{\vttp}{\vtt^{\|}}
\newcommand{\vttf}{ V_{\fisher}}
\newcommand{\vtts}{ V_{\tau\tau,*}}
\newcommand{\vtt}{ V_{\tau\tau}}
\newcommand{\vttn}{ V_{\nm}}
\def\hvtt{\hat V_{\tau\tau}}
\def\hvttP{\hat V_{\tau\tau}^\|}
\def\hvttR{\hat V_{\tau\tau}^\perp}
\def\hvtd{\hat V_{\tau \delta}}
\def\hvdt{\hat V_{\delta\tau }}
\newcommand{\vttl}{ V_{\lin}}
\newcommand{\bsl}{ S_\lin}
\newcommand{\bsf}{ S_\fisher}
\newcommand{\slin}{S_{\lin,qk}}
\newcommand{\sfisher}{S_{\fisher,qk}}




\newcommand{\hY}{\hat Y}
\newcommand{\hbtt}{\hbt_{t}}
 
%
\newcommand{\pr}{{\rm pr}}
\newcommand{\prgn}[1]{\noindent\textbf{#1}}
\newcommand{\prg}[1]{\smallskip\noindent\textbf{#1}}
 \newcommand{\ot}[1]{1, \ldots,#1}
 \newcommand{\zt}[1]{0, 1, \ldots,#1}
 \newcommand{\twot}[1]{2, \ldots,#1}
  

\newcommand{\ehws}{\textsc{ehw} }
\newcommand{\ehw}{\textsc{ehw}} 
\newcommand{\diag}{\textup{diag}} 
\newcommand{\hbg}{\hat{\gamma}}


\newcommand{\vhatehw}{\hat{ V}_\ehw}


\def\bv{(\beta_1, \dots, \beta_Q)}
\newcommand{\betas}{(\bb_q)_{q\in\mt} }
\newcommand{\betais}{(\hat{ \gamma}^\ols_q)}
\newcommand{\betaas}{(\hat{\gamma}_{\textsc{f},\ols})}

\newcommand{\hbYStar}{ \hbY^{( G)}_*(q)}
 
\newcommand{\sg}{span ( g_h)_{h=1}^H }
\newcommand{\bb}{ \beta}
\newcommand{\be}{ \epsilon}





% --------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\CRE}{\textsc{CRE}}
\newcommand{\oY}{\dot{Y}}
\def\T{{ \mathrm{\scriptscriptstyle T} }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\itemc}{\item[$\cdot$]}
\newcommand{\itemq}{\item[$\longrightarrow$] \textbf{Question}:}
\newcommand{\itemtd}{\item[$\longrightarrow$] \textbf{To do}:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\oS}{\dot{ S}}
\newcommand{\tS}{\tilde{ S}}
\newcommand{\bbi}{  \beta^\textsc{l}}
\newcommand{\bba}{  \beta^\textsc{f}}
\newcommand{\hbb}{ \hat{ \beta}}
\newcommand{\hbbstar}{ \hat{ \beta}^*}
\newcommand{\hbbi}{\hat{ \gamma}^\ols}
\newcommand{\hbba}{\hat{\beta}_{\textsc{f},\ols}}
\newcommand{\bbU}{\bar{ U}}
\newcommand{\hbbU}{\hat{{ U}}}
\newcommand{\hbbO}{\hat{{ \Omega}}}
\newcommand{\bbO}{\bar{ \Omega}}
\newcommand{\obbt}{\dot{\bar{ \tau}}}

\newcommand{\cov}{\textup{cov} } 
\newcommand{\var}{\textup{var} } 
\newcommand{\mX}{\mathbb{X}}
\newcommand{\mP}{\mathbb{P}}
\newcommand{\mI}{ I}
\newcommand{\mJ}{\mathbb{J}}
 
\newcommand{\Cp}{{ C_{\perp}}}
\newcommand{\Bp}{{ B^{\perp}}}
\newcommand{\Tp}{{ \Theta^{\perp}}}
\newcommand{\ba}{ \alpha}
%%%%%%%%%%%%%%%%%%%
\newcommand{\bL}{ \Lambda}
 \newcommand{\bTh}{ \Theta}


\def\gg{ \Gamma_G}




 

\newcommand{\hbtStar}{\tilde {\bt}}

\newcommand{\hbtStarQ}{\hbt_*^{(Q-1)}}
\newcommand{\hbtG}{\hbt_{ \Gamma}}
\newcommand{\hbtGG}{\hbt^{( G)}_{ \Gamma}}
\newcommand{\hbtCC}{\hbt^{( C)}_{ \Gamma^\textsc{f}}}




\newcommand{\bth}{  \theta}

\newcommand{\adjwls}{{\fisher,\wls}}
\newcommand{\adjols}{{\fisher,\ols}}

 \newcommand{\hbtfp}{\hbt_\textsc{f}^*}
\newcommand{\hmuadj}{\hat{\mu}_\textsc{f}}
\newcommand{\hbgadjp}{\hat{ \gamma}_\textsc{f}^*}


\newcommand{\all}{{\text{all}}}
\newcommand{\fisher}{\textsc{f}}
\newcommand{\adda}{{\text{adj, all}}}
\newcommand{\addf}{{\text{adj, part}}}
\newcommand{\hbtc}{\hbt_\textsc{c}}
\newcommand{\hbtcols}{\hbt_{\textsc{c},\ols}}
\newcommand{\hbtcwls}{\hbt_{\textsc{c},{\wls}}}
%\newcommand{\tbtFadjols}{\tbt^\textsc{f}_{\mF,\ols}}
%\newcommand{\tbtFadjwls}{\tbt^\textsc{f}_{\mF,\wls}}
%\newcommand{\tmuadj}{\tilde{\mu}_\textsc{f}}
\newcommand{\tmuadjols}{\hat{\mu}_{\textsc{c},\ols}}
\newcommand{\tmuadjwls}{\hat\mu_{\textsc{c},\wls}}
\newcommand{\tbaadjols}{\hat{\ba}_{\textsc{c},\ols}}
\newcommand{\tbaadjwls}{\hat{\ba}_{\textsc{c},\wls}}
\newcommand{\tbbadjols}{\hat{\bb}_{\textsc{c},\ols}}
\newcommand{\tbbadjwls}{\hat{\bb}_{\textsc{c},\wls}}

\newcommand{\bEF}{ E_{\mF}}
\newcommand{\bEt}{ E_{\bt}}
\newcommand{\bEmu}{ E_{\mu}}
\newcommand{\bEa}{ E_{\ba}}


\newcommand{\bWQ}{ W_{1:Q}}
 \newcommand{\bY}{ \bar Y}
\newcommand{\bCF}{ C_{\mF}}
\newcommand{\tbDF}{\tilde{ D}_{\mF}}
 

\newcommand{\ATEi}{\widehat{\text{ATE}}_\textsc{l}}
\newcommand{\ATEa}{\widehat{\text{ATE}}_\textsc{f}}

\newcommand{\cond}{\,\,\left|\,\,}
\newcommand{\toinp}{\overset{p}{\to}}
\newcommand{\td}{\noindent{\tiny\dotfill}}

%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbY}{\bar{ Y}}
\newcommand{\hbY}{\hat{{ Y}}}
\newcommand{\dotsim}{\overset{.}{\sim}}
\newcommand{\proj}{\textup{proj}}
\newcommand{\res}{\textup{res}}






\newcommand{\vttzGamma}{\vtt(\Gamma,z)}
\newcommand{\vttG}{ V_{\tau\tau }^{( G)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mM}{\mathcal{M}}
%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Sigwt}{ \Sigma_{ W \tau}}
\newcommand{\Sigtw}{ \Sigma_{ \tau W}}
\newcommand{\SigWw}{ \Sigma_{ W w}}
\newcommand{\SigwW}{ \Sigma_{ w W}}
%%%%%%%%%%%%%%%%%%
\newcommand{\vttP}{\vtt^{\|}}
\newcommand{\vttR}{\vtt^{\perp}}
\newcommand{\vttRG}{\vtt^{\perp (  G)}}
\newcommand{\vttRO}{\vtt^{\perp (  \Omega)}}
\newcommand{\vttRC}{\vtt^{\perp (  C)}}
\newcommand{\vttRQ}{\vtt^{\perp (\cs)}}
\newcommand{\vttPG}{\vtt^\|( G)}
\newcommand{\vttPB}{\vtt^{\| ( B)}}
 
\newcommand{\vttPQ}{\vtt^{\| \, \cs}}
\newcommand{\vttPC}{\vtt^{\| ( C)}}
\newcommand{\vttPz}{ V_{ \tau \tau,z}^{\| }}
\newcommand{\vttRz}{ V_{ \tau \tau,z}^{\perp }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\vttPzPx}{ V_{ \tau \tau}^{\| z\|  w}}
\newcommand{\vttPzRx}{ V_{ \tau \tau}^{\| z\perp w}}
\newcommand{\vttRzPx}{ V_{ \tau \tau}^{\perp z\| w}}
\newcommand{\vttRzRx}{ V_{ \tau \tau}^{\perp z\perp w}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\vttPGPB}{ V_{ \tau \tau}^{\| G\|  B}}
\newcommand{\vttPGRB}{ V_{ \tau \tau}^{\| G\perp B}}
\newcommand{\vttRGPB}{ V_{ \tau \tau}^{\perp G\| B}}
\newcommand{\vttRGRB}{ V_{ \tau \tau}^{\perp G\perp B}}
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\vttPx}{ V_{ \tau \tau}^{\|  w}}
\newcommand{\vttRx}{ V_{ \tau \tau}^{\perp  w}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\asim}{\overset{\cdot}{\sim}}
\def\assim{\stackrel{\cdot}{=}}
\newcommand{\aperp}{\perp^\infty}
\newcommand{\projw}{\proj_{\hbd}}
\newcommand{\projwC}{\proj_{\hbdC}}
\newcommand{\projz}{\proj_{\hdz }}
\newcommand{\resw}{\res_{\hbd}}
\newcommand{\resz}{\res_{\hdz }}
\newcommand{\Ew}{E_{\hbd}}
\newcommand{\Ez}{E_{\hdz }}
\newcommand{\covw}{\cov_{\hbd}}
\newcommand{\covwC}{\cov_{\hbdC}}
\newcommand{\covz}{\cov_{\hdz }}

\newcommand{\Sxx}{ S_{\delta\delta}}
\newcommand{\Stt}{ S_{ \tau \tau}}
\newcommand{\Stw}{ S_{\tau\delta}}
\newcommand{\Swt}{ S_{\delta\tau}}
\newcommand{\Sqq}{S_{qq}}
\newcommand{\Sqw}{ S_{q w}}
\newcommand{\Swq}{ S_{ w q}}


\newcommand{\Yp}{Y^{\|}}
\newcommand{\Yr}{Y^{\perp}}
\newcommand{\Sp}{S^{\|}}
\newcommand{\Sr}{S^{\perp}}
\newcommand{\vp}{ V^{\|}}
\newcommand{\vr}{ V_\lin}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mK}{\mathcal{K}}
 

\newcommand{\mL}{{\mathcal{L}}}

\newcommand{\mR}{\mathbb{R}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\dbA}{\dot{ G}}

\def\begina{\begin{eqnarray*}}
\def\enda{\end{eqnarray*}}
\def\beginy{\begin{eqnarray}}
\def\endy{\end{eqnarray}}
\def\begine{\begin{enumerate}}
\def\ende{\end{enumerate}}
